A scale-covariant quantum space-time

A noncommutative space-time admitting dilation symmetry was briefly mentioned in the seminal work of Doplicher, Fredenhagen and Roberts. In this paper we explicitly construct the model in details and carry out an in-depth analysis. The C*-algebra that describes this quantum space-time is determined, and it is shown that it admits an action by *-automorphisms of the dilation group, along with the expected Poincar\'e covariance. In order to study the main physical properties of this scale-covariant model, a free scalar neutral field is introduced as a investigation tool. Our key results are then the loss of locality and the irreducibility, or triviality, of special field algebras associated with regions of the ordinary Minkowski space-time. It turns out, in the conclusions, that this analysis allows also to argue on viable ways of constructing a full conformally covariant model for quantum space-time.

==> a1.tex <==
\section{The free fermionic field}

This appendix is devoted to the construction of the Majorana's fermionic field over a generic model of quantum space-time. Towards the end we shall show that the massless fermionic field constructed on the scale-covariant model of quantum space-time is itself scale-covariant as the scalar field discussed in the thesis.

In order to fix the notation we shall collect some basic results, mainly drawn from \cite{weinbergI95}. We recall that the Majorana's fermionic field $\psi$ is such that $\psi=\psi^*$, this being made possible by the existence of a special representation of the Dirac's $\gamma$ matrices, in which each $\gamma$ is pure imaginary. This makes the Dirac's equation real, as well as its solutions, and the classical Majorana's fermionic field operator on the Fock space $\Hilb_F$ can be written as
\begin{equation}\label{eq:majorana}
	\psi(x)=\frac1{(2\pi)^{3/2}}\sum_{\sigma=1}^2\int\left[e^{-ik^\mu x_\mu}a_\sigma(\bv k)\otimes u_\sigma(\bv k) + e^{ik^\mu x_\mu}a_\sigma(\bv k)^*\otimes u_\sigma(\bv k)^*\right]\de\Omega_m^+(\bv k),
\end{equation}
where $\{u_\sigma(\bv k)\in\IC^4,\sigma=1,2\}$ is the set of independent solutions of the momentum equation
\begin{equation}
	(\gamma^\mu_Mp_\mu - m\Id_4)u_\sigma(\bv p) = 0,\qquad p^\mu\ |\ p^0 = \sqrt{\norm{\bv p}^2+m^2}.
\end{equation}
Lorentz covariance on the spinor space $\IC^4$ is implemented by the action of the representation $S:\Lup\to\Mat_{4\times4}(\IC)$ of the proper orthochronous Lorentz group $\Lup$, and is such that
\begin{equation}\label{eq:bridge}
	(\alpha_L\otimes\Id\psi)(x) = (\Id\otimes S(\Lambda^{-1}))\psi(\Lambda x + a),\qquad\forall(\Lambda,a)\in\Pup,
\end{equation}
as required by Wightman's second axiom for quantum field theory. The explicit expression of $S$ can be given in terms of the $\gamma$ matrices, viz.
\begin{equation}
	S(\Lambda) = \exp(-\frac i4\sigma_{\mu\nu}\omega^{\mu\nu}),
\end{equation}
where
  $$\qquad\sigma_{\mu\nu}=\frac i2[\gamma_\mu,\gamma_\nu]\qquad\text{and}\qquad\Lambda = e^{\eta\omega},$$
and this shows that the Majorana's representation $S(\Lambda)$ of $\Lup$ is real for any $\Lambda\in\Lup$.

We recall that the transformation law of the mass-$m$ and spin-$1/2$ one-particle states involves a two-dimensional unitary representation, namely $D:H\to\Mat_{2\times2}(\IC)$ of the stabiliser $H$ of a point $k$ belonging to the orbit associated with the irreducible representation $[m,1/2]$ of the universal covering of the Poincaré subgroup $\tilde\Pup$. Explicitly we have
\begin{equation}
	(\alpha_L\psi_\sigma)(\bv p)=e^{-i(\Lambda p)^\mu a_\mu}\sum_{\bar\sigma=1}^2D(W(\Lambda,p))_{\bar\sigma\sigma}\psi_{\bar\sigma}(\bv p_\Lambda),\qquad(\Lambda,a)\in\Pup,
\end{equation}
where
\begin{equation}
	W(L,p) = L_{\Lambda p}^{-1}\Lambda L_p\in H,\qquad L_p \ |\ p = L_p k,
\end{equation}
which leads directly to the transformation law of the creation and annihilation operators, viz.
\begin{equation}\label{eq:spinor_annihilator}
	\alpha_L a_\sigma(\bv k) = e^{i(\Lambda p)^\mu a_\mu}\sum_{\bar\sigma=1}^2D(W(\Lambda,p)^{-1})_{\sigma\bar\sigma}a_{\bar\sigma}(\bv p_\Lambda).
\end{equation}

We may exploit equation \eqref{eq:bridge} in order to establish a relation between the representations $S$ and $D$. Introducing the explicit action \eqref{eq:spinor_annihilator} in the left-hand side of \eqref{eq:bridge} we determine
\begin{equation}
	S(\Lambda)u_\sigma(\bv k) = \sum_{\bar\sigma=1}^2D(W(\Lambda,p)^{-1})_{\bar\sigma\sigma}u_{\bar\sigma}(\bv k_\Lambda).
\end{equation}

Before proceeding to the construction of the field on quantum space-time we shall recall one more property of the fermionic field $\psi$, regarding its scaling behaviour. For the sake of dimensional analysis only, we recall the structure of the action for the field $\psi$, which is
\begin{equation}
	\mathcal S[\psi] \approx \int m\overline\psi(x) \psi(x)\de^4x,
\end{equation}
$m$ being a mass and thus having the physical dimensions of an energy. We infer from this that the physical dimensions in terms of energy of the field $\psi$ are
\begin{equation}
	D_{\psi} = \frac32.
\end{equation}





\subsection{Construction of the field}

Let us consider a quantum space-time described by the \calg\ $\mathcal E$, and let $q_\mu$, $\mu=0,\ldots,1$ stand for a representation of the commutation relations among the coordinates. Using von Neumann's definition of non commutative functional calculus \eqref{eq:vnncc} we may define the Majorana field on quantum space-time in the same way as the scalar field \eqref{eq:scalar_field}, namely
\begin{align}\label{eq:spinor}
	\psi(q) = \frac1{(2\pi)^{3/2}}\sum_{\sigma=1}^2\int&\big[e^{-ik^\mu q_\mu}\otimes a_\sigma(\bv k)\otimes u_\sigma(\bv k)\nonumber\\
		&+ e^{ik^\mu q_\mu}\otimes a_\sigma(\bv k)^*\otimes u_\sigma(\bv k)^*\big]\de\Omega_m^+(\bv k),
\end{align}
$\psi(q)$ being an element of the tensor product $\mathcal E\otimes\Bound(\Hilb_F)\otimes\IC^4$. Using the definition \eqref{eq:derivative} of derivative, we can verify that the field \eqref{eq:spinor} satisfies the Dirac's equation
\begin{subequations}
\begin{equation}
	(i\tilde\gamma^\mu_M\partial_\mu-m\tilde\Id)\psi(q)=0,
\end{equation}
where
\begin{equation}
	\tilde\gamma^\mu_M = \Id\otimes\Id\otimes\gamma^\mu_M\qquad\text{and}\qquad\tilde\Id=\Id\otimes\Id\otimes\Id.
\end{equation}
\end{subequations}

In order to define the map $\mathcal S(\mathcal E)\mapsto\Bound(\Hilb_F)$, we notice from the definition \eqref{eq:spinor} of the field that we need to take 4-tuples of states $\omega\in\mathcal S(\mathcal E)^{\times 4}$ and define the pairing
\begin{equation}\label{eq:pairing}
	\langle\ \cdot\ ,\ \cdot\ ):\mathcal S(\mathcal E)^{\times 4}\times \IC^4\to\IC
\end{equation}
such that
\begin{equation}
	\left\langle\omega(e^{ik^\mu q_\mu}), u_\sigma(\bv k)\right) = \sum_{k=1}^4\omega_k(e^{ik^\mu q_\mu})u_\sigma(\bv k)_k.
\end{equation}
Thus we may set
\begin{align}
	\psi(\omega) = \frac1{(2\pi)^{3/2}}\sum_{\sigma=1}^2\int&\Big[\left\langle\omega(e^{-ik^\mu q_\mu}),u_\sigma(\bv k)\right) a_\sigma(\bv k)\nonumber\\
		&+ \left\langle\omega(e^{ik^\mu q_\mu}),u_\sigma(\bv k)^*\right)  a_\sigma(\bv k)^*\Big]\de\Omega_m^+(\bv k),
\end{align}
for each $\omega\in\mathcal S(\mathcal E)^{\times 4}$, and we may introduce the four functions $\psi_\omega(x)$ associated with the four states $\omega$ in the usual way (cf. \eqref{eq:psi}), i.e.
\begin{equation}
	\varphi_\omega(x) = \frac1{(2\pi)^4}\int e^{ik^\mu x_\mu}\omega(e^{-ik^\mu q_\mu})\de^4k.
\end{equation}
Taking the Fourier transform of the remaining terms and extending the pairing \eqref{eq:pairing} by linearity we end up with the more familiar expression
\begin{equation}\label{eq:sd}
	\psi(\omega)=\int\left\langle\varphi_\omega(x),\psi(x)\right)\de^4x,
\end{equation}
with $\psi(x)$ being the ordinary Majorana field \eqref{eq:majorana} defined on classical space-time.





\subsection{Covariance}

Let us start the analysis of the property of covariance of the fermionic field \eqref{eq:spinor} by considering the action of the Poincaré group $\Pup$. As in the case of the scalar field, we shall again use $\tau_L$ and $\alpha_L$ to denote the automorphisms on $\mathcal E$ and $\Bound(\Hilb_F)$ respectively. Recalling formulae \eqref{eq:tau_on_q}, \eqref{eq:spinor_annihilator} and \eqref{eq:sd} we find
\begin{align*}
	(\tau_L^{-1}\otimes\alpha_L^{-1}\otimes S(\Lambda)^{-1})\psi(q) &= \psi(q),
\end{align*}
%\frac1{(2\pi)^{3/2}}\sum_{\sigma=1}^2\int&\big[e^{-ik^\mu(\Lambda q + a\Id)_\mu}\otimes e^{-ik^\mu a_\mu}\sum_{\bar\sigma=1}^2D(W(\Lambda,p))_{\sigma\bar\sigma}a_{\bar\sigma}(\bv k_\Lambda)\otimes S(\Lambda)^{-1}u_\sigma(\bv k)+\hc]\de\Omega_m^+(\bv k),
which proves the Poincaré covariance of the field.

We now restrict our attention to the massless case on the scale-covariant model of quantum space-time in order to implement the covariance under dilations. To this end we first recall a basic fact from relativistic kinematic regarding the motion of a massless particle. It is well known that the momentum $\bv p$ of a body whose motion is described by the 4-momentum $p^\mu$ satisfying $p^\mu p_\mu = 0$ can be rescaled by an arbitrary factor $\lambda\in\IR^+$ by a suitable choice of a boost along the direction of $\bv p$\footnote{If we were considering photons, we would call this the \emph{relativistic Doppler effect}.}. To see this, consider a massless particle travelling along the $x^1$ direction, e.g. $p=(\norm{\bv p},\norm{\bv p},0,0)$, and the boost
\begin{equation}
	B_{\beta,\hv p} = \begin{bmatrix}\gamma &-\gamma\beta\\-\gamma\beta & \gamma\end{bmatrix}\oplus\Id_2.
\end{equation}
The new 4-momentum $p'$ is thus given by $B_{\beta,\hv p}p$, viz.
\begin{equation}
	p' = \lambda p,\qquad\lambda = \sqrt{\frac{1-\beta}{1+\beta}},
\end{equation}
which gives the relation $\beta=\beta(\lambda)$ between the boost parameter $\beta$ and the scaling factor $\lambda$. We now only define the two families automorphisms on the $a_\sigma(\bv k)$s and the $u_\sigma(\bv k)$s respectively
\begin{subequations}
\begin{align}
	\delta_\lambda^{-1} a_\sigma(\bv k) &= \lambda^{\frac12}\sum_{\bar\sigma=1}^2D(W(B_{\beta(\lambda),\hv k}^{-1},k))_{\sigma\bar\sigma}a_{\bar\sigma}(\lambda\bv k),\\
	\mathfrak d_\lambda^{-1}u_\sigma(\bv k) &= S(B_{\beta(\lambda),\hv k})u_\sigma(\bv k),
\end{align}
\end{subequations}
for we already have the action \eqref{eq:tdilation} on the coordinates $q$ of the scale-covariant model of quantum space-time. Hence using \eqref{eq:sd} again we verify that
\begin{equation}
	(\Delta_\lambda^{-1}\otimes\delta_\lambda^{-1}\otimes\mathfrak d_\lambda^{-1})\psi(q) = \frac1{\lambda^{3/2}}\psi(q),
\end{equation}
which expresses the expected behaviour.


==> a2.tex <==
\section{Grassmann algebras\label{app:grassmann}}

In this appendix we shall introduce some concepts drawn from the theory of Grassmann algebras in order to fix the notation and to \emph{intrinsically} construct an automorphism on the Grassmann algebra on the classical Minkowski space-time that occurs frequently in the main body of the thesis.

We recall that on a (pseudo-)Riemannian manifold $(M,g)$ there exists a natural isomorphism between the vector spaces $T_pM$ and $T^*_pM$, for any $p\in M$, given by the metric structure of $M$: the map
\begin{equation}
	v \mapsto \iota_v g
\end{equation}
is a bijection from $T_pM$ to $T^*_pM$ for any $v\in T_pM$ and $p\in M$.

We shall also recall the definition of the \emph{reciprocal} or \emph{dual} basis. Let $(M,g)$ be a (pseudo-)Riemannian manifold of dimension $n$, and let $\{e_1,\ldots,e_n\}$ be a basis for $T_pM$, $p\in M$. Then there exists a unique basis $\{e_*^1,\ldots,e_*^n\}$ of $T^*_pM$ such that
\begin{equation}
	e_*^i(e_k) = g(e_i,e_k).
\end{equation}
Such a basis is called \emph{reciprocal} or \emph{dual} to $\{e_1,\ldots,e_n\}$.

For a more comprehensive treatment of the arguments discussed in this appendix and for some of the proofs of the following results, we refer to textbooks on the subject, such as e.g. \cite{nakahara03}.

\subsection{Main definitions and results}

In this section we shall employ the symbol $V$ to denote a generic real vector space of finite dimension $n\in \IN$, and $V^*$ to denote its algebraic dual space, i.e. the space of all the linear functionals $\Hom(V,\IR)$ on $V$.

Let $\Ant\in\End\left(\bigoplus_{k=0}^n\bigotimes^k V^*\right)$ denote the antisymmetriser, i.e. the projection given by
\begin{equation}
	(\Ant\omega^p)(v_1,\ldots,v_p) := \frac1{p!}\sum_{\sigma\in\mathscr S_p}\sgn(\sigma)\omega^p(v_{\sigma(1)},\ldots,v_{\sigma(p)}),
\end{equation}
for any $\omega^p\in\bigotimes^p V^*$ and $v_1,\ldots,v_p\in V$, $k=0,\ldots,n$, $\mathscr S_p$ being the symmetric group of order $p!$. As a consequence of the definition, each vector space $\bigotimes^pV^*$ is $\Ant$-stable, i.e.
\begin{equation}
	\Ran\Ant\at_{\bigotimes^pV^*}\subset{\bigotimes}^pV^*,\qquad\forall p\in\{0,\ldots,n\}.
\end{equation}

\begin{definition}[$p$-form space] The subset
	\begin{equation}
		\bw^pV^*:=\Ran\Ant\at_{\bigotimes^p V^*},\qquad p\in{0,\ldots,n}
	\end{equation}
	of $\bigotimes^p V^*$ is called the \emph{$p$-form space} on $V$.
\end{definition}

The limitation of $p$ to $\{0,\ldots,n\}$ is due to the fact that the range of the restriction of $\Ant$ on $\bigotimes^pV^*$ is always the trivial subspace $\{0\}$ for any $p>n$.
\begin{theorem}\label{thm:pform} Each $p$-form space $\bw^pV^*$, $p\in\{0,\ldots,n\}$, is a vector subspace of $\bigotimes^pV^*$ of dimension $\binom np$.\end{theorem}

Let $\bws V^*$ be the vector space obtained by taking the direct sum of all the $p$-form spaces $\bw^pV^*$ on $V$, namely
\begin{equation}
	\bws V^* := \bigoplus_{k=0}^n\bw^kV^*.
\end{equation}
We now define the \emph{exterior product} on $\bws V^*$, i.e. the map $\wedge:\bws V^*\times\bws V^*\to\bws V^*$ given by
\begin{align}
	(\omega^p\wedge\eta^q)&(v_1,\ldots, v_{p+q})\nonumber\\
		&:= \frac1{p!q!}\sum_{\sigma\in\mathscr S_{p+q}}\omega^p(v_{\sigma(1)},\ldots,v_{\sigma(p)})\eta^q(v_{\sigma(p+1)},\ldots,v_{\sigma(p+q)}),
\end{align}
for any $p$-form $\omega^p$ and $q$-form $\eta^q$ naturally embedded in $\bws V^*$, and $v_1,\ldots,v_{p+q}\in V$, $p+q\leq n$.
\begin{theorem} The vector space $\bws V^*$ endowed with the multiplication law $\wedge$ is an algebra.\end{theorem}
As a consequence of this result we now give the following
\begin{definition}[Grassmann algebra] The triple $(\bws V^*,+,\wedge)$ is called the \emph{Grassmann} or \emph{exterior algebra} on $V$.\end{definition}

The determinant of a linear map $A\in\End(V^*)$ may be defined intrinsically, i.e. independent on the basis of $V^*$. Let $\tilde A\in\End(\bws V^*)$ be the map given by
\begin{equation}
	\tilde A(\alpha_1 \wedge\cdots\wedge \alpha_p) := (A\alpha_1)\wedge\cdots\wedge(A\alpha_p),\qquad\forall \alpha_1,\ldots,\alpha_p\in V^*,
\end{equation}
for any $p\in\{0,\ldots,n\}$. Theorem \ref{thm:pform} asserts that $\dim\bw^nV^*=1$, and therefore there must exists a real number $c(A)\in\IR$ depending on $A$ such that
\begin{equation}
	\tilde A\Omega = c(A)\Omega,
\end{equation}
where $\Omega$ is any basis element of $\bw^nV^*$. It turns out that, if $\det(A)$ denotes the determinant of the matrix associated with $A$ expressed in an arbitrary basis of $V^*$, then
\begin{equation}\label{eq:determinant}
	c(A)\equiv\det(A).
\end{equation}





\subsection{The map between ``$\sigma_0$'' and ``$\sstd$''}

Let $(M,\eta)$ be a pseudo-Riemannian manifold, with $M=\IR^4$ and $\eta\in\Bil(M)$ the Minkowski pseudo-metric. Our aim is to define a map $A\in\Aut\left(\bws M^*\right)$ such that
\begin{subequations}\label{eq:A_props}
\begin{equation}
	\Ran A\at_{\bw^kM^*}\subset \bw^kM^*,\qquad \forall k\in\{0,\ldots,n\},
\end{equation}
and
\begin{equation}
	(A\sigma_0)(u,v)=\sstd(u,v),\quad\forall u,v\in M,
\end{equation}
\end{subequations}
where $\sigma_0,\sstd\in\bw^2M$ have been defined in chapter \ref{chap:model}, equations \eqref{eq:sigma0} and \eqref{eq:sstd} respectively. To this end we take an automorphism $a\in\Aut(M^*)$ and define the action of $A$ on the subspace $M^*$ of $\bws M^*$ by means of
\begin{equation}
	A\alpha := a\alpha,\qquad\forall\alpha\in M^*.
\end{equation}
This allows us to extend  $A$ to the whole $\bws M^*$ by simply considering the transpose of $a$, i.e. the automorphism $\widetilde a\in\Aut(M)$ such that
\begin{equation}
	(A\alpha)(v) = \alpha(\tilde av),\qquad \forall \alpha\in M^*, v\in M,
\end{equation}
depending on the metric structure of $M$, namely
\begin{equation}
	\alpha(\tilde av)=\eta^{-1}(\alpha, A\iota_v\eta),\qquad\forall a\in M^*,v\in M.
\end{equation}
The notion of $\tilde a$ may be used to extend the action of $A$ on $\bws M^*$ in such a way that
\begin{equation}
	(A\omega^k)(v_1,\ldots,v_k):=\omega^k(\tilde av_1,\ldots,\tilde av_k)
\end{equation}
for any $\omega^k\in\bw^kM^*$ and $v_1,\ldots v_k\in M$, $k=0,2,\ldots,4$. Thus the first property in \eqref{eq:A_props} is satisfied.

We now consider both the canonical basis $\{e_0,\ldots,e_3\}$ of $M$ and the action of $A$ on $\sigma_0$. We have
\begin{align*}
	(A\sigma_0)(u,v) &= \sigma_0(\tilde au,\tilde av)\\
		&= (\sigma_0)_{\mu\nu}(\tilde au)^\mu(\tilde av)^\nu\\
		&= (\sstd)_{\mu\nu}u^\mu v^\nu,
\end{align*}
and thus
\begin{equation}
	[\sstd] = [a][\sigma_0][a]^T,
\end{equation}
for a suitable choice of the matrix $[a]$ associated with $a$, $[\sstd]$ and $[\sigma_0]$ denoting the matrices of coefficients of $\sstd$ and $\sigma_0$ in the canonical reciprocal basis $\{e_*^0,\ldots,e_*^3\}$ of $M$, i.e. those given by \eqref{eq:sstd} and \eqref{eq:sigma0_mat} respectively. Such a matrix $[a]$, which concretely defines the action $A$ on $\bws M^*$, exists, an explicit expression may be found in \cite{perini} and it turns out that
\begin{equation*}
	A(e_*^0\wedge\cdots\wedge e_*^3) = -e_*^0\wedge\cdots\wedge e_*^3,
\end{equation*}
i.e.
\begin{equation}
	\det(A)=\det(a) = -1.
\end{equation}
However we may completely ignore the explicit form of the matrix, which is \cite{perini}
\begin{equation}\label{eq:A_matrix}
  A=\begin{bmatrix}0&1&0&0\\1&0&0&0\\0&0&1&0\\1&0&0&1\end{bmatrix}
\end{equation}
for the automorphism $A$ has been intrinsically defined on $\bws M$, its main purpose being that of allowing to switch from geometrical objects depending on $\sigma_0$ to those depending on $\sstd$, and vice-versa. We may express this intrinsic action by the formal expressions
\begin{equation}
	A\text{``}\sigma_0\text{''} = \text{``}{\sstd}\text{''}\qquad\iff\qquad A^{-1}\text{``}\sstd\text{''} = \text{``}{\sigma_0}\text{''},
\end{equation}
and we can extend $A$ to elements of $M$ by setting
\begin{equation}
	\alpha(Av) := \eta^{-1}(\alpha,A\iota_v\eta),\qquad\forall v\in M,\alpha\in M^*,
\end{equation}
for no confusion may arise provided one let $A$ act according to its argument.

\begin{lemma}\label{lem:auto} Let $\eta:V\times V\to \IR$ be a symmetric and non-degenerate bilinear form on $V$, $T\in\Aut(V)$ and $\tilde T$ the map such that
\begin{equation}
	(\tilde T\omega^k)(v_1,\ldots,v_k) := \omega^k(Tv_1,\ldots,Tv_k),
\end{equation}
for any $\omega^k\in\otimes^k V^*$ and $v_1,\ldots,v_k\in V$, $k\in\IN$. Then the map $T^\dagger:V\to V$ given by
\begin{equation}
	\alpha(T^\dagger v) := \eta^{-1}(\alpha,\iota_{T^{-1}v}(T\eta)),\qquad\forall\alpha\in V^*,v\in V,
\end{equation}
is an automorphism.
\end{lemma}
\begin{proof}
Since $\eta$ is non-degenerate, it suffice to prove that $v\mapsto\iota_{T^{-1}v}(T\eta)$ is an isomorphism between $V$ and $V^*$. Since $T$ is an automorphism, $T\eta$ is a non-degenerate and symmetric bilinear form, and therefore the map $u\mapsto \iota_u(T\eta)$ is an isomorphism between $V$ and $V^*$. Hence $v\mapsto\iota_{T^{-1}v}(T\eta)$ is the composition between an automorphism on $V$, namely $T^{-1}$, and an isomorphism between $V$ and $V^*$.
\end{proof}
We now extend further the action of $A$ on the bilinear forms $\phi\in\Bil(M)$ on $M$ by means of
\begin{equation}
	(A\phi)(u,v) := \phi(Au,Av),\qquad\forall u,v\in M.
\end{equation}
According to all the above definitions, we then have the following identity
\begin{equation}\label{eq:bil_id}
	\phi(u,v)=(A^{-1}\phi)(Au,Av),\qquad\forall\phi\in\Bil(M),u,v\in M,
\end{equation}
which, in conjunction with lemma \ref{lem:auto}, allows us to prove the following
\begin{theorem}\label{thm:dagger} For any $A\in\Aut(M)$ there exists an $A^\dagger\in\Aut(M)$ such that
\begin{equation}
	\eta(u, Av) = \eta(A^\dagger u, v),\qquad\forall u,v \in M.
\end{equation}
\end{theorem}
\begin{proof} Using the identity \eqref{eq:bil_id} we find
\begin{align*}
	\eta(u,Av) &= (A\eta)(A^{-1}u, v)\\
		&= \left(\iota_{A^{-1}u}(A\eta)\right)(v)\\
		&= \eta(\iota_{\iota_{A^{-1}u}(A\eta)}\eta^{-1},v),
\end{align*}
and according to lemma \ref{lem:auto}, the map
\begin{equation}
	u\mapsto\iota_{\iota_{A^{-1}u}(A\eta)}\eta^{-1},\qquad u\in M,
\end{equation}
is an automorphism, say $u\mapsto A^\dagger u$, $A^\dagger\in\Aut(M)$ and $u\in M$. Therefore we have
\begin{equation}
	\eta(u,Av)=\eta(A^\dagger u,v),\qquad A^\dagger\in\Aut(M),
\end{equation}
which proves the assertion.
\end{proof}

